Type-Preserving Flow Analysis and Interprocedural Unboxing (Extended Version)

Interprocedural flow analysis can be used to eliminate otherwise unnecessary heap allocated objects (unboxing), and in previous work we have shown how to do so while maintaining correctness with respect to the garbage collector. In this paper, we extend the notion of flow analysis to incorporate types, enabling analysis and optimization of typed programs. We apply this typed analysis to specify a type preserving interprocedural unboxing optimization, and prove that the optimization preserves both type and GC safety along with program semantics. We also show that the unboxing optimization can be applied independently to separately compiled program modules, and prove via a contextual equivalence result that unboxing a module in isolation preserves program semantics.

==> abstract.tex <==
Interprocedural flow analysis can be used to eliminate otherwise
unnecessary heap allocated objects (\emph{unboxing}), and in previous
work we have shown how to do so while maintaining correctness with
respect to the garbage collector.  In this paper, we extend the notion
of flow analysis to incorporate types, enabling analysis and
optimization of typed programs.  We apply this typed analysis to
specify a type preserving interprocedural unboxing optimization, and
prove that the optimization preserves both type and GC safety along
with program semantics.  We also show that the unboxing optimization
can be applied independently to separately compiled program modules,
and prove via a contextual equivalence result that unboxing a module
in isolation preserves program semantics.



==> introduction.tex <==
Many languages and compilers use a \emph{uniform object
representation} in which every source level object is represented at
least initially by a heap allocated object.  Such a representation
allows polymorphic functions to be compiled once and enables the
implementation of features that use runtime type information.  In this
representation machine integers and floating-point numbers are placed
in a single-field object, a box, and this operation is called boxing.
Operations such as addition require first projecting the number from
the box (unboxing), followed by the actual addition, followed by the
creation of a new box for the result (boxing).  Boxing and unboxing
operations add considerable overhead, and thus it is highly desirable
to remove them when possible -- e.g. when polymorphism or features
requiring runtime type information are not being used.  We refer to
the general class of optimizations that attempt to remove unnecessary
box and unbox operations as \emph{unboxing} optimizations.  We refer
to unboxing optimizations that attempt to eliminate boxing and
unboxing across function boundaries as \emph{interprocedural
unboxing}.  We also include in this latter category optimizations
(such as the one given in this paper) which attempt to unbox objects
written to and read from other objects in the heap.

Interprocedural unboxing presents additional challenges in a typed
setting, since type information must be updated to reflect any
unboxing.  A box might flow to an argument in an application, and the
parameter of the called function might flow to an unbox operation.  If
the optimization decides to remove the box and unbox operations then
it must also remove the box type on the parameter.  In other words,
typed unboxing requires not just rewriting uses and definitions in the
traditional sense, but also rewriting intermediate points in the
program through which the unboxed values flow.  At a high level then,
the optimization can be viewed as selecting a set of box operations,
unbox operations, and box types to remove.  Such a selection has a
global consistency requirement---a box type should only be removed if
all boxes that flow to it are removed, a box operation should only be
removed if all unbox operations it flows to are removed, and so on.
Thus choosing a set of boxed objects to eliminate and rewriting the
program to reflect this choice in a consistent manner requires knowing
what things flow to what points in the program, a question that flow
analyses are designed to answer.  In this paper we use the results of
flow analysis to formulate correctness conditions for unboxing and
then prove that those conditions ensure correct optimization.

In previous work~\cite{Petersen:2012} we considered a simpler problem,
that of rewriting garbage-collector (GC) metadata rather than full
types.  An accurate GC requires specifying for each field of each
object and each slot of each stack activation frame whether it
contains a pointer into the GC heap or not (contains a machine
integer, floating-point number, etc.).  As with types, when
interprocedurally unboxing such metadata must be rewritten in a
globally consistent manner.  Our previous paper showed how to do this
rewriting correctly using the results of a flow analysis, in a whole
program setting.  In this paper we extend these ideas to develop a
methodology for dealing with interprocedural optimization of
statically typed languages (including universal polymorphism) in a
type preserving fashion.  We also show that this methodology does not
depend on whole program compilation, and extends easily to support
modular compilation.

In the following sections, we begin by defining a core language with a
polymorphic type system that has box and unbox operations.  As in our
previous paper we formalize a notion of GC safety for our
language---that the GC metadata is currently correct---and show that
well-typed programs are GC safe throughout execution.  Next we specify
a set of abstract conditions that a reasonably flow analysis must
satisfy, with the property that any flow analysis that satisfies these
conditions can be used in our framework to optimize programs.  The
main section of the paper defines an unboxing optimization
parameterized over a choice of objects to unbox, and gives a set of
correctness conditions under which such a choice is guaranteed to
preserve typing and preserve semantics.  We show that this set of
correctness conditions is satisfiable by constructing a simple
unboxing algorithm which satisfies these conditions. Finally we extend
the system slightly by defining a notion of unboxing for modules and
show that it is correct in the sense that a module is contextually
equivalent to its unboxing.

While our paper is specifically about the concrete optimization of
unboxing, the ideas used here generalize naturally to other
optimizations that change the representation of objects in a non-local
fashion.  For example, dead-field elimination and dead-parameter
elimination impose similar requirements for rewriting types and GC
metadata in a globally consistent fashion.  Flow analyses can be used
to specify and implement these (and others), and we believe (based on
practical experience in our compiler) that the framework presented
here extends naturally to such optimizations.  As far as we know, this
and our previous paper are the first to use a flow analysis to rewrite
types and GC metadata in a globally consistent fashion, and to use a
flow analysis to formulate correctness conditions for this rewriting
process and prove these conditions sound.

\omitthis{
Precise garbage collection (\emph{GC}) for managed languages is usually
implemented by requiring the compiler to keep track of meta-data
indicating which variables and fields contain GC-managed references
and which should be ignored by the garbage collector. We refer to this
information as the \emph{traceability} of a field or variable: a field
or variable is traceable if it should be treated as a pointer into the
heap by the garbage collector.  

In order to maintain this information in the presence of polymorphic
functions (including subtype polymorphism), many languages and
compilers use a \emph{uniform object representation} in which every
source level object is represented at least initially by a heap
allocated object.  All interprocedural use of native (non-heap) data
therefore occurs only through fields of objects.  This is commonly
referred to as \emph{boxing}, objects represented in this way are
referred to as \emph{boxed}, and projecting out of the uniform
representation is referred to as
\emph{unboxing}.  Boxing imposes substantial performance penalties for
many reasons: the additional overhead of the allocation and projection
is substantial, arrays of boxed objects exhibit poor locality, and the
additional memory pressure can cause bottlenecks in the hardware.  

In previous work\cite{Petersen:2012}, we showed how to use the results
of interprocedural flow analyses (e.g. pointer analysis or reaching
definitions) to implement an interprocedural unboxing optimization
while preserving the meta-data necessary for precise garbage
collection.  The core language targeted by the flow analysis in that
paper was untyped.  In this paper, we extend our framework to target a
strongly typed polymorphic core language, and develop a typed unboxing
optimization.  We show that under suitable correctness criteria, our
optimization always maps well-typed programs to well-typed programs.
To the best of our knowledge, this is first work to extend flow
analysis to the type level and to use this to do interprocedural
optimizations in a type-preserving fashion.

In the following sections, we define a type-safe high-level core
language, and show that the types capture essential aspects of GC
meta-data and GC safety.  We then give a high-level specification of
what a reasonable flow analysis on this language must compute,
extending this to the type level. We define a notion of a general
unboxing optimization for this language, and give a specification for
when such an optimization is acceptable for a given flow analysis.  We
show that the optimization induced by an acceptable unboxing preserves
the semantics of the original program, including type (and therefore
GC) safety.  Finally, we construct an algorithm closely based on one
in use in our compiler and prove that it produces an unboxing that
satisfies our correctness specification, and hence that it preserves
the semantics of the program (including GC safety).
}
\iftr
\else
All the lemmas and theorems in the paper have been proven.  Proofs are
available in an extended technical report~\cite{Glew:2012:extended}.
\fi


==> paper-specific-macros.tex <==
\long\def\omitthis#1{}

\newcommand{\kwbox}{\kwop{box}}
\newcommand{\kwunbox}{\kwop{unbox}}

\newcommand{\kwlet}{\kwop{let}}
\newcommand{\kwin}{\kwop{in}}

\newcommand{\labelof}[1]{\mathrm{lbl}(#1)}
\newcommand{\labelsin}[1]{\mathrm{lbls}(#1)}
\newcommand{\Lbld}[2]{{#1}^{#2}}
\newcommand{\LbldP}[2]{{(#1)}^{#2}}

\newcommand{\tybase}{\kwop{B}}
\newcommand{\tyfun}[3]{\forall#1.#2\rightarrow#3}
\newcommand{\tybox}[1]{\kwbox(#1)}
\newcommand{\tytotr}[1]{\mathit{tr}(#1)}

\newcommand{\EMLet}[2]{\begin{cascade}
                          \kwlet \cascitem
                             #1 \cascback{1}
                          \kwin #2
                        \end{cascade}}
\newcommand{\ELet}[2]{\kwlet\ #1\ \kwin #2}

\newcommand{\EBox}[2]{\kwbox_{#1}{#2}}
\newcommand{\VBox}[2]{\langle {#2};{#1}\rangle }
\newcommand{\EUnbox}[1]{\kwunbox #1}
\newcommand{\ELam}[3]{\lambda#1;#2.#3}
\newcommand{\EFix}[6]{\kwop{fix}\;#1[#2](#3;#4);#5.#6}
\newcommand{\VLam}[4]{\langle#1,\lambda#2;#3.#4\rangle}
\newcommand{\VFix}[7]{\langle#1,\kwop{fix}\;#2[#3](#4;#5);#6.#7\rangle}
\newcommand{\EApp}[3]{#1[#2]\;#3}
\newcommand{\VConst}{c}

\newcommand{\LEBox}[3]{\LbldP{{\mathtt{box}}_{#1}{\, #2}}{#3}}
\newcommand{\LVBox}[3]{\Lbld{\langle {#2};{#1}\rangle}{#3}}
\newcommand{\LEUnbox}[2]{\LbldP{\kwunbox #1}{#2}}
\newcommand{\LELam}[4]{\LbldP{\lambda#1;#2.#3}{#4} }
\newcommand{\LEFix}[7]{\LbldP{\EFix{#1}{#2}{#3}{#4}{#5}{#6}}{#7}}
\newcommand{\LEApp}[4]{\LbldP{\EApp{#1}{#2}{#3}}{#4}}
\newcommand{\LVLam}[5]{\Lbld{\langle#1,\lambda#2;#3.#4\rangle}{#5}}
\newcommand{\LVFix}[8]{\Lbld{\VFix{#1}{#2}{#3}{#4}{#5}{#6}{#7}}{#8}}
\newcommand{\LVConst}[1]{\Lbld{c}{#1}}

\newcommand{\TBits}{\kw{b}}
\newcommand{\TRef}{\kw{r}}
\newcommand{\subst}[3]{{#1}[#2/#3]}
\newcommand{\T}{\mathrm{T}}
\newcommand{\TOpt}{\underline{\T}}
\newcommand{\U}{\Upsilon}
\newcommand{\A}{\mathrm{A}}
\newcommand{\cache}{\mathrm{C}}
\newcommand{\env}{\rho}
\newcommand{\benv}{\varrho}
\newcommand{\bind}[4]{#1;#2=\Lbld{#3}{#4}}
\newcommand{\unboxes}[3]{\down{#1}^{#2}_{#3}}
\newcommand{\unboxesTU}[1]{\unboxes{#1}{}{\U}}
%\newcommand{\unboxesTU}[1]{\unboxes{#1}{\T}{\U}}
\newcommand{\unboxesv}[3]{\unboxes{#1}{#2}{#3}}
\newcommand{\unboxesvTU}[1]{\unboxesTU{#1}}

\newcommand{\traceable}[1]{\vdash #1\ \mathrm{\bf tr}}
\newcommand{\traceablev}[2]{\vdash_{\mathrm{v}} #1;#2}

\newcommand{\agrees}[1]{\stackrel{#1}{\simeq}}
\newcommand{\agreesU}{\agrees{\U}}
\newcommand{\agreesTU}{\agrees{\T, \U}}

\newcommand{\consistent}[2]{#1\vdash#2}
\newcommand{\consistentt}[3]{#1\vdash#2:#3}
\newcommand{\consistentU}[1]{\consistent{\U}{#1}}
\newcommand{\consistentUt}[2]{\consistentt{\U}{#1}{#2}}

\newcommand{\cacheConsistent}[2]{#1 \vdash #2}
\newcommand{\cacheConsistentCU}{\cacheConsistent{\cache}{\U}}
\newcommand{\cacheConsistentCTU}{\cacheConsistent{\cache}{(\T, \U)}}


\newcommand{\good}[5]{#1 \vdash #5 \downharpoonleft \downharpoonright (#3, #4)}
\newcommand{\goodv}[5]{#1 \vdash_\textrm{v} #5\ \downharpoonleft \downharpoonright\ (#3, #4)}
\newcommand{\goodTU}[3]{\good{#1}{#2}{\T}{\U}{#3}}
\newcommand{\goodvTU}[3]{\goodv{#1}{#2}{\T}{\U}{#3}}
\newcommand{\goodCETU}[1]{\goodTU{\cache}{\benv}{#1}}
\newcommand{\goodvCETU}[1]{\goodvTU{\cache}{\benv}{#1}}

\newcommand{\analysis}[3]{#1\semi #2 \vdash #3}
\newcommand{\analysisC}[1]{\cache\vdash#1}
\newcommand{\analysisCE}[1]{\analysis{\cache}{\benv}{#1}}
\newcommand{\analysisv}[2]{#1\vdash_{v} #2}
\newcommand{\analysisvC}[1]{\analysisv{\cache}{#1}}

\newcommand{\sanalysis}[3]{#1\semi #2 \vdash^{\sf s} #3}
\newcommand{\sanalysisCE}[1]{\sanalysis{\cache}{\benv}{#1}}

\newcommand{\instantiates}[4]{#1\semi #2 \vdash #3 \,\leadsto\, #4}
\newcommand{\instantiatesCE}[2]{\instantiates{\cache}{\benv}{#1}{#2}}

\newcommand{\instantiatesv}[4]{#1\semi #2 \vdash_v #3 \,\leadsto\, #4}
\newcommand{\instantiatesvCE}[2]{\instantiatesv{\cache}{\benv}{#1}{#2}}
\newcommand{\dfd}[1]{\textrm{def}(#1)}
\newcommand{\undfd}[1]{\textrm{undef}(#1)}

\newcommand{\CC}{\mathcal{CC}}
\newcommand{\EC}{\mathcal{EC}}
\newcommand{\THat}{\mathcal{T}}
\newcommand{\THatHat}{\THat_{\EC}}
\newcommand{\UHat}{\mathcal{U}}
\newcommand{\that}{\hat{t}}
\newcommand{\cand}{\mathcal{CN}}
\newcommand{\lub}{\sqcup}
\newcommand{\itr}{\mathit{itr}}

\newcommand{\ms}[2]{(#1,#2)}

\newcommand{\SConst}[2]{\Lbld{#1}{#2}}
\newcommand{\STyBase}[1]{\Lbld{\tybase}{#1}}
\newcommand{\SLam}[4]{\LbldP{\forall#1.#2\rightarrow#3}{#4}_{\sf v}}
\newcommand{\STyFun}[4]{\LbldP{\forall#1.#2\rightarrow#3}{#4}_{\sf t}}
\newcommand{\SBox}[3]{\LEBox{#1}{#2}{#3}_{\sf v}}
\newcommand{\STyBox}[2]{\LEBox{}{#1}{#2}_{\sf t}}

\newcommand{\EMPTY}{\epsilon}

\usepackage{theorem}
\theoremstyle{break}
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newtheorem{observation}{Observation}

\semicolonforbindingcolon
\ltgtforanglebrackets

\newcommand{\tjM}[2]{\vdash#1:#2}
\newcommand{\tjMod}[1]{\vdash#1\;\mathit{wf}}
\newcommand{\tjE}[2]{\vdash#1:#2}
\newcommand{\tje}[3]{#1\vdash#2:#3}
\newcommand{\tjC}[4]{#1\vdash#2:\substhole{#3}{#4}}
\newcommand{\tjt}[2]{#1\vdash#2\;\mathit{wf}}
\newcommand{\tjeq}[2]{\vdash#1=#2}
\newcommand{\ftv}[1]{\mathit{ftv}(#1)}
\newcommand{\tctxt}[2]{#1\semi#2}

\newcommand{\funcond}[4]{\mathit{funC}(#1,#2,#3,#4)}
\newcommand{\boxcond}[2]{\mathit{boxC}(#1,#2)}

\newcommand{\module}[3]{(#1\Rightarrow#2:#3)}
\newcommand{\notunboxed}[2]{#1\vdash#2\;\mathit{not\;unboxed}}
\newcommand{\notunboxedU}[1]{\notunboxed{\U}{#1}}

\newcommand{\lr}[1]{[\![#1]\!]}
\newcommand{\lrv}[2]{\lr{#1}^{\sf v}_{#2}}
\newcommand{\lre}[2]{\lr{#1}^{\sf e}_{#2}}
\newcommand{\lrE}[1]{\lr{#1}^{\sf E}}
\newcommand{\lenv}{\psi}
\newcommand{\lrequiv}[4]{#1\vdash#2\equiv#3:#4}

\newcommand{\ctxteqe}[4]{#1\vdash#2\equiv#3:#4}
\newcommand{\ctxteqM}[2]{\vdash#1\equiv#2}
\newcommand{\obseq}[2]{#1\stackrel{\it obs}{\equiv}#2}
\newcommand{\substhole}[2]{#1\langle#2\rangle}
\newcommand{\hole}{\langle\rangle}

\newcommand{\IFF}{\Leftrightarrow}

\newcommand{\uirM}[3]{\cache\semi\benv\semi\U\vdash_{\sf uir}^{\sf M}#1\equiv#2:#3}
\newcommand{\uirE}[3]{\cache\semi\benv\semi\U\vdash_{\sf uir}^{\sf E}#1\equiv#2:#3}
\newcommand{\uire}[4]{\cache\semi\benv\semi\U\semi#1\vdash_{\sf uir}^{\sf e}#2\equiv#3:#4}

\newcommand{\unboxmetric}[1]{\delta(#1)}
\newcommand{\restrict}[2]{#1\downharpoonright#2}
\newcommand{\synequiv}{\sim_{\sf s}}


==> related.tex <==
This paper provides a modular approach to showing correctness of a
realistic compiler optimization that rewrites the structure of
program data structures in significant ways.  Our approach uses an
arbitrary inter-procedural reaching definitions analysis to eliminate
unnecessary heap allocation in an intermediate representation in which
object representation has been made explicit.  Our optimization can be
staged freely with other optimizations.  Unlike any previous work
that we are aware of, we account for correctness with respect to the
meta-data requirements of the garbage collector.  For presentational
purposes, we have restricted our attention to the core concern of GC
safety, but additional issues such as value size, dynamic type tests,
etc. are straightforward to incorporate.

There has been substantial previous work addressing the problem of
unboxing.  Peyton Jones \cite{Jones91unboxedvalues} introduced an
explicit distinction between boxed and unboxed objects to provide a
linguistic account of unboxing, and hence to allow a high-level
compiler to locally eliminate unboxes of syntactically apparent box
introduction operations.  Leroy \cite{Leroy:1992:UOP:143165.143205}
defined a type-driven approach to adding coercions into and out of
specialized representations.  The type driven translation represented
monomorphic objects natively (unboxed, in our terminology), and then
introduced wrappers to coerce polymorphic uses into an appropriate
form.  To a first-order approximation, instead of boxing at definition
sites this approach boxes objects at polymorphic use sites.  This
style of approach has the problem that it is not necessarily
beneficial, since allocation is introduced in places where it would
not otherwise be present.  This is reflected in the slowdowns observed
on some benchmarks described in the original paper.  This approach
also has the potential to introduce space leaks.  In a later paper
\cite{Leroy97theeffectiveness} Leroy argued that a simple untyped
approach gives better and more predictable results.

Henglein and J{\o}rgensen \cite{Henglein:1994:FOB:174675.177874}
defined a formal notion of optimality for local unboxings and gave two
different choices of coercion placements that satisfy their notion of
optimality.  Their definition of optimality explicitly does not
correspond in any way to reduced allocation or reduced instruction
count and does not seem to provide uniform improvement over Leroy's
approach.  

The MLton compiler \cite{Weeks:2006:WCM:1159876.1159877} largely
avoids the issue of a uniform object representation by completely
monomorphizing programs before compilation.  This approach requires
whole-program compilation.  More limited monomorphization schemes
could be considered in an incremental compilation setting.
Monomorphization does not eliminate the need for boxing in the
presence of dynamic type tests or reflection.  Just in time compilers
(e.g. for .NET) may monomorphize dynamically at runtime.

The TIL compiler
\cite{harper+:intensional,Tarditi:2004:TTO:989393.989449} uses
intensional type analysis in a whole-program compiler to allow native
data representations without committing to whole-program compilation.
As with the Leroy coercion approach, polymorphic uses of objects
require conditionals and boxing coercions to be inserted at use sites,
and consequently there is the potential to slow down, rather than
speed up, the program.

Serrano and Feeley \cite{Serrano:1996:SUA:232627.232635} described a
flow analysis for performing unboxing substantially similar in spirit
to our approach.  Their algorithm attempts to find a monomorphic
typing for a program in which object representations have not been
made explicit, which they then use selectively to choose whether to
use a uniform or non-uniform representation for each particular
object.  Their approach differs in that they define a dedicated
analysis rather than using a generic reaching definitions analysis.
They assume a conservative garbage collector and hence do not need to
account for the requirements of GC safety, and they do not prove a
correctness result.

